Co-Attention for Conditioned Image Matching

We propose a new approach to determine correspondences between image pairs in the wild under large changes in illumination, viewpoint, context, and material. While other approaches find correspondences between pairs of images by treating the images independently, we instead condition on both images to implicitly take account of the differences between them. To achieve this, we introduce (i) a spatial attention mechanism (a co-attention module, CoAM) for conditioning the learned features on both images, and (ii) a distinctiveness score used to choose the best matches at test time. CoAM can be added to standard architectures and trained using self-supervision or supervised data, and achieves a significant performance improvement under hard conditions, e.g. large viewpoint changes. We demonstrate that models using CoAM achieve state of the art or competitive results on a wide range of tasks: local matching, camera localization, 3D reconstruction, and image stylization.

==> attentioncoamfigure.tex <==
\begin{figure*}[h]
    \begin{minipage}{\linewidth}
        \centering
        \begin{overpic}[width=0.9\linewidth]{attn1.png}
        \put(-3,19){\footnotesize $I^1$}
        \put(-3,11){\footnotesize $I^2$}
        \put(-3,3){\footnotesize $A$}
        \end{overpic}
        \vspace{0.5em}
    \end{minipage} 
        \caption{{\bf CoAM Attention.} Here we visualise the predicted attention ($A$) for sample image pairs. The point for which we visualise the attention is shown as a red dot in $I^1$. While it is not clear apriori what the attention module should do precisely, we can see that it does attend to relevant, similar regions in the other image and is dependent on the query location.}
        \label{fig:attentioncoamresults}
\end{figure*}

==> sfmresults.tex <==
\begin{table*}[t]
    \centering
    \caption{{\bf SfM.} We compare our approach to using SIFT features on 3D reconstruction for two datasets: Large SfM and Sculpture. Both are collections of images from the web containing large variations in illumination and viewpoint. These metrics are a proxy for 3D reconstruction quality, so we encourage the reader to view the reconstructions in the supplementary. X: failure. $\uparrow$: higher is better. $\downarrow$: lower is better. \textcolor{blue}{\bf blue}: best result.}
    \scriptsize
    \begin{tabular}{@{}crccccccccccccc@{}}
    \toprule
                & & \multicolumn{3}{c}{Large SfM} & \multicolumn{9}{c}{Sculpture Dataset } \\
                \cmidrule{3-5} \cmidrule{7-15}
         \multicolumn{2}{r}{\bf Landmark:} &  MM  & Gen & Tow & & HM1 & HM2 & HM3 & HM4 & HM5 & HM6 & HM7 & HM8 & HM9 \\
         \multicolumn{2}{r}{\# Images:} & 1344  & 1463 & 1576 & & 12 & 124 & 250 & 266 & 78 & 31 & 358 & 238 & 74 \\
         

    \midrule
    \multirow{2}{*}[0pt]{\# Reg.~Ims $\uparrow$} & {\bf SIFT \cite{Lowe04}:} & 500 & 1035 & 804 & & X & 103 & \textcolor{blue}{\bf 198} & 212 & 61 & 22 & 266 & \textcolor{blue}{\bf 201} & 53  \\
        & {\bf Ours:} & \textcolor{blue}{\bf 702} & \textcolor{blue}{\bf 1072} & \textcolor{blue}{\bf 967} & & \textcolor{blue}{\bf 12} & \textcolor{blue}{\bf 108} & 194 & \textcolor{blue}{\bf 215} & \textcolor{blue}{\bf 67} & \textcolor{blue}{\bf 25} & \textcolor{blue}{\bf 284} & \textcolor{blue}{\bf 201} & \textcolor{blue}{\bf 57}  \\ \midrule
    \multirow{2}{*}[0pt]{\# Sparse Pts $\uparrow$} & {\bf SIFT \cite{Lowe04}:} & 116K & 338K & 239K & & X & 48K & 70K & 102K & 28K & 9K & 128K & \textcolor{blue}{\bf 99K} & \textcolor{blue}{\bf 23K} \\
    & {\bf Ours: } & \textcolor{blue}{\bf 256K} & \textcolor{blue}{\bf 570K} & \textcolor{blue}{\bf 452K} & & \textcolor{blue}{\bf 2.9K} & \textcolor{blue}{\bf 63K} & \textcolor{blue}{\bf 83K} & \textcolor{blue}{\bf 121K} & \textcolor{blue}{\bf 40K} & \textcolor{blue}{\bf 10K} & \textcolor{blue}{\bf 190K} & \textcolor{blue}{\bf 99K} & 21K \\ \midrule
    
    \multirow{2}{*}[0pt]{Track Len $\uparrow$} & {\bf SIFT \cite{Lowe04}:} & \textcolor{blue}{\bf 6.32} & 5.52 & \textcolor{blue}{\bf 7.76} & & X & \textcolor{blue}{\bf 5.33} & \textcolor{blue}{\bf 5.92} & \textcolor{blue}{\bf 5.80} & \textcolor{blue}{\bf 4.54} & \textcolor{blue}{\bf 4.73} & \textcolor{blue}{\bf 4.46} & \textcolor{blue}{\bf 5.24} & 4.75 \\
    & {\bf Ours: } & 6.09 & \textcolor{blue}{\bf 6.60} & 5.82 & & \textcolor{blue}{\bf 3.60} & 5.03 & 5.43 & 5.61 & 4.32 & 4.00 & 4.23 & \textcolor{blue}{\bf 5.24} & \textcolor{blue}{\bf 4.77} \\ \midrule
    
    \multirow{2}{*}[0pt]{Reproj Err (px) $\downarrow$} & {\bf SIFT \cite{Lowe04}:} & \textcolor{blue}{\bf 0.60} & \textcolor{blue}{\bf 0.69} & \textcolor{blue}{\bf 0.61} & & X & 1.31 & 1.32 & \textcolor{blue}{\bf 1.28} & 1.30 & 1.33 & \textcolor{blue}{\bf 1.22} & \textcolor{blue}{\bf 1.30} & \textcolor{blue}{\bf 1.32} \\
    & {\bf Ours: } & 1.30 & 1.34 & 1.32 & & \textcolor{blue}{\bf 1.33} & \textcolor{blue}{\bf 1.30} & \textcolor{blue}{\bf 1.30} & 1.29 & \textcolor{blue}{\bf 1.29} & \textcolor{blue}{\bf 1.26} & 1.23 & \textcolor{blue}{\bf 1.30} & \textcolor{blue}{\bf 1.32} \\ \midrule
    
    \multirow{2}{*}[0pt]{\# Dense Pts $\uparrow$} & {\bf SIFT \cite{Lowe04}:} & \textcolor{blue}{\bf 1.8M} & \textcolor{blue}{\bf 4.2M} & \textcolor{blue}{\bf 3.1M} & & X & 160K & 143K & \textcolor{blue}{\bf 307K} & 73K & \textcolor{blue}{\bf 46K} & 174K & 333K & \textcolor{blue}{\bf 54K} \\
    & {\bf Ours: } & 1.1M & 2.1M & 1.8M & & \textcolor{blue}{\bf 0.2K} & \textcolor{blue}{\bf 188K} & \textcolor{blue}{\bf 156K} & 296K & \textcolor{blue}{\bf 82K} & 44K & \textcolor{blue}{\bf 187K} & \textcolor{blue}{\bf 333K} & 53K \\
    
         
    \bottomrule
    \end{tabular}
    \label{tab:reconstructionresults}
\end{table*}



==> stylisation_results.tex <==
\begin{figure*}
    \begin{minipage}{\linewidth}
        \centering
        \begin{overpic}[width=0.9\linewidth]{figure.png}
        \put(-6,5){\footnotesize \cite{Luan17}}
        \put(-6,20){\footnotesize Ours}
        \put(-6,35){\footnotesize GT$_S$}
        \put(-8,48){\footnotesize Inputs}
        \put(-8,45){\footnotesize ($I_v$, $I_s$)}
        \put(5,-2){\footnotesize (a)}
        \put(20,-2){\footnotesize (b)}
        \put(35,-2){\footnotesize (c)}
        \put(49,-2){\footnotesize (d)}
        \put(64,-2){\footnotesize (e)}
        \put(79,-2){\footnotesize (f)}
        \put(93,-2){\footnotesize (g)}
        \end{overpic}
        \vspace{0.5em}
    \end{minipage} 
        \caption{{\bf Stylization.} Given $I_s$ and $I_v$, the task is to generate an image with the pose and viewpoint of $I_v$ and style of $I_s$. We show results for \modelname~and a baseline that uses semantics \cite{Luan17}. We also show the resampled image (GT$_S$) which is computed using the true correspondences from the MegaDepth dataset \cite{Li18}.
        While \cite{Luan17} works well for easy cases, it sometimes copies style from $I_v$ (as shown by the red background in (a), unlit building in (b), and red hued building in (g)). \cite{Luan17} also fails if the semantic prediction is incorrect (e.g.~(c) and (e)).}
        \label{fig:stylisationresults}
\end{figure*}
